The distribution of open clusters in the Galaxy

In this work we explore the new catalog of galactic open clusters that became available recently, containing 1750 clusters that have been re-analysed using the Gaia DR2 catalog to determine the stellar memberships. We used the young open clusters as tracers of spiral arms and determined the spiral pattern rotation speed of the Galaxy and the corotation radius, the strongest Galactic resonance. The sample of open clusters used here increases the last one from Dias et al. (2019) used in the previous determination of the pattern speed by dozens objects. In addition, the distances and ages values are better determined, using improvements to isochrone fitting and including an updated extinction polynomial for the Gaia DR2 photometric band-passes, and the Galactic abundance gradient as a prior for metallicity. In addition to the better age determinations, the catalog contains better positions in the Galactic plane and better proper motions. This allow us to discuss not only the present space distribution of the clusters, but also the space distribution of the clusters's birthplaces, obtained by integration of the orbits for a time equal to their age. The value of the rotation velocity of the arms ($28.5 \pm 1.0$ km s$^{-1}$ kpc$^{-1}$) implies that the corotation radius ($R_c$) is close to the solar Galactic orbit ($R_c/R_0 = 1.01\pm0.08$), which is supported by other observational evidence discussed in this text. A simulation is presented, illustrating the motion of the clusters in the reference frame of corotation. We also present general statistics of the catalog of clusters, like spatial distribution, distribution relative to height from the Galactic plane, and distribution of ages and metallicity. An important feature of the space distribution, the corotation gap in the gas distribution and its consequences for the young clusters, is discussed.

==> refs2.tex <==
@ARTICLE{Koda16,
       author = {{Koda}, Jin and {Scoville}, Nick and {Heyer}, Mark},
        title = "{Evolution of Molecular and Atomic Gas Phases in the Milky Way}",
      journal = {ApJ},
     keywords = {evolution, Galaxy: disk, Galaxy: evolution, ISM: atoms, ISM: clouds, ISM: molecules, Astrophysics - Astrophysics of Galaxies},
         year = 2016,
        month = jun,
       volume = {823},
       number = {2},
          eid = {76},
        pages = {76},
          doi = {10.3847/0004-637X/823/2/76},
archivePrefix = {arXiv},
       eprint = {1604.01053},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...823...76K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dambis15,
       author = {{Dambis}, A.~K. and {Berdnikov}, L.~N. and {Efremov}, Yu. N. and {Kniazev}, A. Yu. and {Rastorguev}, A.~S. and {Glushkova}, E.~V. and {Kravtsov}, V.~V. and {Turner}, D.~G. and {Majaess}, D.~J. and {Sefako}, R.},
        title = "{Classical Cepheids and the spiral structure of the milky way}",
      journal = {Astronomy Letters},
     keywords = {Galactic structure, Cepheids, spiral arms, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = sep,
       volume = {41},
       number = {9},
        pages = {489-500},
          doi = {10.1134/S1063773715090017},
archivePrefix = {arXiv},
       eprint = {1505.01782},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015AstL...41..489D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{FehZhightgrad,
       author = {{Li}, Chengdong and {Zhao}, Gang and {Zhai}, Meng and {Jia}, Yunpeng},
        title = "{The Formation and Evolution of Galactic Disks with APOGEE and the Gaia Survey}",
      journal = {ApJ},
     keywords = {Galaxy: disk, Galaxy: evolution, Galaxy: kinematics and dynamics, Galaxy: structure, methods: data analysis, stars: abundances},
         year = 2018,
        month = jun,
       volume = {860},
       number = {1},
          eid = {53},
        pages = {53},
          doi = {10.3847/1538-4357/aac50f},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...860...53L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chen2001,
       author = {{Chen}, Bing and {Stoughton}, Chris and {Smith}, J. Allyn and {Uomoto}, Alan and {Pier}, Jeffrey R. and {Yanny}, Brian and {Ivezi{\'c}}, {\v{Z}}eljko and {York}, Donald G. and {Anderson}, John E. and {Annis}, James and {Brinkmann}, Jon and {Csabai}, Istv{\'a}n and {Fukugita}, Masataka and {Hindsley}, Robert and {Lupton}, Robert and {Munn}, Jeffrey A. and {SDSS Collaboration}},
        title = "{Stellar Population Studies with the SDSS. I. The Vertical Distribution of Stars in the Milky Way}",
      journal = {ApJ},
     keywords = {Galaxy: Stellar Content, Galaxy: Structure},
         year = 2001,
        month = may,
       volume = {553},
       number = {1},
        pages = {184-197},
          doi = {10.1086/320647},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001ApJ...553..184C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Skowron2019,
       author = {{Skowron}, Dorota M. and {Skowron}, Jan and {Mr{\'o}z}, Przemek and {Udalski}, Andrzej and {Pietrukowicz}, Pawe{\l} and {Soszy{\'n}ski}, Igor and {Szyma{\'n}ski}, Micha{\l} K. and {Poleski}, Rados{\l}aw and {Koz{\l}owski}, Szymon and {Ulaczyk}, Krzysztof and {Rybicki}, Krzysztof and {Iwanek}, Patryk},
        title = "{A three-dimensional map of the Milky Way using classical Cepheid variable stars}",
      journal = {Science},
     keywords = {ASTRONOMY, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = aug,
       volume = {365},
       number = {6452},
        pages = {478-482},
          doi = {10.1126/science.aau3181},
archivePrefix = {arXiv},
       eprint = {1806.10653},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019Sci...365..478S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Joshi2007MNRAS.378..768J,
       author = {{Joshi}, Y.~C.},
        title = "{Displacement of the Sun from the Galactic plane}",
      journal = {MNRAS},
     keywords = {methods: statistical, astronomical data bases: miscellaneous, open clusters and associations: general, Galaxy: structure, Astrophysics},
         year = 2007,
        month = jun,
       volume = {378},
       number = {2},
        pages = {768-776},
          doi = {10.1111/j.1365-2966.2007.11831.x},
archivePrefix = {arXiv},
       eprint = {0704.0950},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007MNRAS.378..768J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Bonatto2006A&A...446..121B,
       author = {{Bonatto}, C. and {Kerber}, L.~O. and {Bica}, E. and {Santiago}, B.~X.},
        title = "{Probing disk properties with open clusters}",
      journal = {A\&A},
     keywords = {Galaxy: open clusters and associations: general, Galaxy: structure, Astrophysics},
         year = 2006,
        month = jan,
       volume = {446},
       number = {1},
        pages = {121-135},
          doi = {10.1051/0004-6361:20053573},
archivePrefix = {arXiv},
       eprint = {astro-ph/0509804},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006A&A...446..121B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Amores2005,
       author = {{Am{\^o}res}, E.~B. and {L{\'e}pine}, J.~R.~D.},
        title = "{Models for Interstellar Extinction in the Galaxy}",
      journal = {AJ},
     keywords = {ISM: Dust, Extinction, Galaxy: Structure, ISM: Clouds, ISM: Structure, Stars: Distances},
         year = 2005,
        month = aug,
       volume = {130},
       number = {2},
        pages = {659-673},
          doi = {10.1086/430957},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005AJ....130..659A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Amores2013,
       author = {{Am{\^o}res}, E.~B. and {L{\'o}pez-Corredoira}, M. and {Gonz{\'a}lez-Fern{\'a}ndez}, C. and {Moitinho}, A. and {Minniti}, D. and {Gurovich}, S.},
        title = "{The long bar as seen by the VVV Survey. II. Star counts}",
      journal = {A\&A},
     keywords = {ISM: structure, dust, extinction, Galaxy: stellar content, Galaxy: structure, Galaxy: center, Galaxy: general, Astrophysics - Astrophysics of Galaxies},
         year = 2013,
        month = nov,
       volume = {559},
          eid = {A11},
        pages = {A11},
          doi = {10.1051/0004-6361/201219846},
archivePrefix = {arXiv},
       eprint = {1308.6022},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013A&A...559A..11A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{BailerJones2009,
       author = {{Bailer-Jones}, C.~A.~L.},
        title = "{The evidence for and against astronomical impacts on climate change and mass extinctions: a review}",
      journal = {International Journal of Astrobiology},
     keywords = {climate change, cosmic rays, hypothesis testing, mass extinctions, minor body impacts, period detection, solar motion, spiral arms, time series analysis, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Astrophysics of Galaxies, Physics - Geophysics, Quantitative Biology - Populations and Evolution},
         year = 2009,
        month = jul,
       volume = {8},
       number = {3},
        pages = {213-219},
          doi = {10.1017/S147355040999005X},
archivePrefix = {arXiv},
       eprint = {0905.3919},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009IJAsB...8..213B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Barros2016,
       author = {{Barros}, D.~A. and {L{\'e}pine}, J.~R.~D. and {Dias}, W.~S.},
        title = "{Models for the 3D axisymmetric gravitational potential of the Milky Way galaxy. A detailed modelling of the Galactic disk}",
      journal = {A\&A},
     keywords = {Galaxy: disk, Galaxy: fundamental parameters, Galaxy: kinematics and dynamics, Galaxy: structure, methods: numerical, methods: statistical, Astrophysics - Astrophysics of Galaxies},
         year = 2016,
        month = sep,
       volume = {593},
          eid = {A108},
        pages = {A108},
          doi = {10.1051/0004-6361/201527535},
archivePrefix = {arXiv},
       eprint = {1607.02541},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016A&A...593A.108B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Barros2013,
       author = {{Barros}, D.~A. and {L{\'e}pine}, J.~R.~D. and {Junqueira}, T.~C.},
        title = "{A Galactic ring of minimum stellar density near the solar orbit radius}",
      journal = {MNRAS},
     keywords = {stars: kinematics and dynamics, Galaxy: evolution, Galaxy: structure, Astrophysics - Astrophysics of Galaxies},
         year = 2013,
        month = nov,
       volume = {435},
       number = {3},
        pages = {2299-2321},
          doi = {10.1093/mnras/stt1454},
archivePrefix = {arXiv},
       eprint = {1308.0627},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MNRAS.435.2299B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{Barford1985,
       author = {{Barford}, N.~C.},
        title = "{Experimental measurements: Precision, error and truth}",
         year = 1985,
         publisher = {Chichester: Wiley, 1985, 2nd ed.},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1985empe.book.....B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Carrera2019,
       author = {{Carrera}, R. and {Bragaglia}, A. and {Cantat-Gaudin}, T. and {Vallenari}, A. and {Balaguer-N{\'u}{\~n}ez}, L. and {Bossini}, D. and {Casamiquela}, L. and {Jordi}, C. and {Sordo}, R. and {Soubiran}, C.},
        title = "{Open clusters in APOGEE and GALAH. Combining Gaia and ground-based spectroscopic surveys}",
      journal = {A\&A},
     keywords = {stars: abundances, open clusters and associations: general, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = mar,
       volume = {623},
          eid = {A80},
        pages = {A80},
          doi = {10.1051/0004-6361/201834546},
archivePrefix = {arXiv},
       eprint = {1901.09302},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...623A..80C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dias2021,
       author = {{Dias}, W.~S. and {Monteiro}, H. and {L{\'e}pine}, J.~R.~D. and {Barros}, D.~A.},
        title = "{Updated parameters of 1758 open clusters based on Gaia DR2}",
      journal = {MNRAS},
     keywords = {Galaxy: kinematics and dynamics, Galaxy: structure, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2021,
        month = submitted,
       volume = {486},
       number = {4},
        pages = {5726-5736},
          doi = {},
    adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Dias2019,
       author = {{Dias}, W.~S. and {Monteiro}, H. and {L{\'e}pine}, J.~R.~D. and {Barros}, D.~A.},
        title = "{The spiral pattern rotation speed of the Galaxy and the corotation radius with Gaia DR2}",
      journal = {MNRAS},
     keywords = {Galaxy: kinematics and dynamics, Galaxy: structure, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = jul,
       volume = {486},
       number = {4},
        pages = {5726-5736},
          doi = {10.1093/mnras/stz1196},
archivePrefix = {arXiv},
       eprint = {1905.08133},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.486.5726D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Dias2014,
   author = {{Dias}, W.~S. and {Monteiro}, H. and {Caetano}, T.~C. and {L{\'e}pine}, J.~R.~D. and 
	{Assafin}, M. and {Oliveira}, A.~F.},
    title = "{Proper motions of the optically visible open clusters based on the UCAC4 catalog}",
  journal = {A\&A},
 keywords = {open clusters and associations: general},
     year = 2014,
    month = apr,
   volume = 564,
      eid = {A79},
    pages = {A79},
      doi = {10.1051/0004-6361/201323226},
   adsurl = {http://adsabs.harvard.edu/abs/2014A%26A...564A..79D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Dias2005,
       author = {{Dias}, Wilton S. and {L{\'e}pine}, J.~R.~D.},
        title = "{Direct Determination of the Spiral Pattern Rotation Speed of the Galaxy}",
      journal = {ApJ},
     keywords = {Galaxy: Disk, Galaxy: Kinematics and Dynamics, Astrophysics},
         year = 2005,
        month = aug,
       volume = {629},
       number = {2},
        pages = {825-831},
          doi = {10.1086/431456},
archivePrefix = {arXiv},
       eprint = {astro-ph/0503083},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005ApJ...629..825D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dias2002,
       author = {{Dias}, W.~S. and {Alessi}, B.~S. and {Moitinho}, A. and {L{\'e}pine}, J.~R.~D.},
        title = "{New catalogue of optically visible open clusters and candidates}",
      journal = {A\&A},
     keywords = {galaxy: open clusters and associations: general, catalogs, Astrophysics},
         year = 2002,
        month = jul,
       volume = {389},
        pages = {871-873},
          doi = {10.1051/0004-6361:20020668},
archivePrefix = {arXiv},
       eprint = {astro-ph/0203351},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002A&A...389..871D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ferreira2020,
       author = {{Ferreira}, F.~A. and {Corradi}, W.~J.~B. and {Maia}, F.~F.~S. and {Angelo}, M.~S. and {Santos}, J.~F.~C., Jr.},
        title = "{Discovery and astrophysical properties of Galactic open clusters in dense stellar fields using Gaia DR2}",
      journal = {MNRAS},
     keywords = {Surveys, open clusters and associations: general, Galaxy: stellar content, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = jun,
       volume = {496},
       number = {2},
        pages = {2021-2038},
          doi = {10.1093/mnras/staa1684},
archivePrefix = {arXiv},
       eprint = {2006.05611},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.496.2021F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{CastroGinard2019,
       author = {{Castro-Ginard}, A. and {Jordi}, C. and {Luri}, X. and {Cantat-Gaudin}, T. and {Balaguer-N{\'u}{\~n}ez}, L.},
        title = "{Hunting for open clusters in Gaia DR2: the Galactic anticentre}",
      journal = {A\&A},
     keywords = {surveys, open clusters and associations: general, astrometry, methods: data analysis, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = jul,
       volume = {627},
          eid = {A35},
        pages = {A35},
          doi = {10.1051/0004-6361/201935531},
archivePrefix = {arXiv},
       eprint = {1905.06161},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...627A..35C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{CastroGinard2020,
       author = {{Castro-Ginard}, A. and {Jordi}, C. and {Luri}, X. and {{\'A}lvarez Cid-Fuentes}, J. and {Casamiquela}, L. and {Anders}, F. and {Cantat-Gaudin}, T. and {Mongui{\'o}}, M. and {Balaguer-N{\'u}{\~n}ez}, L. and {Sol{\`a}}, S. and {Badia}, R.~M.},
        title = "{Hunting for open clusters in Gaia DR2: 582 new open clusters in the Galactic disc}",
      journal = {A\&A},
     keywords = {surveys, open clusters and associations: general, astrometry, methods: data analysis, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = mar,
       volume = {635},
          eid = {A45},
        pages = {A45},
          doi = {10.1051/0004-6361/201937386},
archivePrefix = {arXiv},
       eprint = {2001.07122},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&A...635A..45C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{cantat2018,
       author = {{Cantat-Gaudin}, T. and {Jordi}, C. and {Vallenari}, A. and
         {Bragaglia}, A. and {Balaguer-N{\'u}{\~n}ez}, L. and {Soubiran}, C. and
         {Bossini}, D. and {Moitinho}, A. and {Castro-Ginard}, A. and
         {Krone-Martins}, A. and {Casamiquela}, L. and {Sordo}, R. and
         {Carrera}, R.},
        title = "{A Gaia DR2 view of the open cluster population in the Milky Way}",
      journal = {A\&A},
     keywords = {stars: distances, Galaxy: disk, Galaxy: structure, open clusters and associations: general, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = oct,
       volume = {618},
          eid = {A93},
        pages = {A93},
          doi = {10.1051/0004-6361/201833476},
archivePrefix = {arXiv},
       eprint = {1805.08726},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018A&A...618A..93C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{CantatGaudin2020,
       author = {{Cantat-Gaudin}, T. and {Anders}, F. and {Castro-Ginard}, A. and {Jordi}, C. and {Romero-G{\'o}mez}, M. and {Soubiran}, C. and {Casamiquela}, L. and {Tarricq}, Y. and {Moitinho}, A. and {Vallenari}, A. and {Bragaglia}, A. and {Krone-Martins}, A. and {Kounkel}, M.},
        title = "{Painting a portrait of the Galactic disc with its stellar clusters}",
      journal = {A\&A},
     keywords = {open clusters and associations: general, Galaxy: disk, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = aug,
       volume = {640},
          eid = {A1},
        pages = {A1},
          doi = {10.1051/0004-6361/202038192},
archivePrefix = {arXiv},
       eprint = {2004.07274},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&A...640A...1C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{GaiaCollab2018,
       author = {{Gaia Collaboration} and {Brown}, A.~G.~A. and {Vallenari}, A. and {Prusti}, T. and {de Bruijne}, J.~H.~J. and {Babusiaux}, C. and {Bailer-Jones}, C.~A.~L. and {Biermann}, M. and {Evans}, D.~W. and {Eyer}, L. and {Jansen}, F. and {Jordi}, C. and {Klioner}, S.~A. and {Lammers}, U. and {Lindegren}, L. and {Luri}, X. and {Mignard}, F. and {Panem}, C. and {Pourbaix}, D. and {Randich}, S. and {Sartoretti}, P. and {Siddiqui}, H.~I. and {Soubiran}, C. and {van Leeuwen}, F. and {Walton}, N.~A. and {Arenou}, F. and {Bastian}, U. and {Cropper}, M. and {Drimmel}, R. and {Katz}, D. and {Lattanzi}, M.~G. and {Bakker}, J. and {Cacciari}, C. and {Casta{\~n}eda}, J. and {Chaoul}, L. and {Cheek}, N. and {De Angeli}, F. and {Fabricius}, C. and {Guerra}, R. and {Holl}, B. and {Masana}, E. and {Messineo}, R. and {Mowlavi}, N. and {Nienartowicz}, K. and {Panuzzo}, P. and {Portell}, J. and {Riello}, M. and {Seabroke}, G.~M. and {Tanga}, P. and {Th{\'e}venin}, F. and {Gracia-Abril}, G. and {Comoretto}, G. and {Garcia-Reinaldos}, M. and {Teyssier}, D. and {Altmann}, M. and {Andrae}, R. and {Audard}, M. and {Bellas-Velidis}, I. and {Benson}, K. and {Berthier}, J. and {Blomme}, R. and {Burgess}, P. and {Busso}, G. and {Carry}, B. and {Cellino}, A. and {Clementini}, G. and {Clotet}, M. and {Creevey}, O. and {Davidson}, M. and {De Ridder}, J. and {Delchambre}, L. and {Dell'Oro}, A. and {Ducourant}, C. and {Fern{\'a}ndez-Hern{\'a}ndez}, J. and {Fouesneau}, M. and {Fr{\'e}mat}, Y. and {Galluccio}, L. and {Garc{\'\i}a-Torres}, M. and {Gonz{\'a}lez-N{\'u}{\~n}ez}, J. and {Gonz{\'a}lez-Vidal}, J.~J. and {Gosset}, E. and {Guy}, L.~P. and {Halbwachs}, J. -L. and {Hambly}, N.~C. and {Harrison}, D.~L. and {Hern{\'a}ndez}, J. and {Hestroffer}, D. and {Hodgkin}, S.~T. and {Hutton}, A. and {Jasniewicz}, G. and {Jean-Antoine-Piccolo}, A. and {Jordan}, S. and {Korn}, A.~J. and {Krone-Martins}, A. and {Lanzafame}, A.~C. and {Lebzelter}, T. and {L{\"o}ffler}, W. and {Manteiga}, M. and {Marrese}, P.~M. and {Mart{\'\i}n-Fleitas}, J.~M. and {Moitinho}, A. and {Mora}, A. and {Muinonen}, K. and {Osinde}, J. and {Pancino}, E. and {Pauwels}, T. and {Petit}, J. -M. and {Recio-Blanco}, A. and {Richards}, P.~J. and {Rimoldini}, L. and {Robin}, A.~C. and {Sarro}, L.~M. and {Siopis}, C. and {Smith}, M. and {Sozzetti}, A. and {S{\"u}veges}, M. and {Torra}, J. and {van Reeven}, W. and {Abbas}, U. and {Abreu Aramburu}, A. and {Accart}, S. and {Aerts}, C. and {Altavilla}, G. and {{\'A}lvarez}, M.~A. and {Alvarez}, R. and {Alves}, J. and {Anderson}, R.~I. and {Andrei}, A.~H. and {Anglada Varela}, E. and {Antiche}, E. and {Antoja}, T. and {Arcay}, B. and {Astraatmadja}, T.~L. and {Bach}, N. and {Baker}, S.~G. and {Balaguer-N{\'u}{\~n}ez}, L. and {Balm}, P. and {Barache}, C. and {Barata}, C. and {Barbato}, D. and {Barblan}, F. and {Barklem}, P.~S. and {Barrado}, D. and {Barros}, M. and {Barstow}, M.~A. and {Bartholom{\'e} Mu{\~n}oz}, S. and {Bassilana}, J. -L. and {Becciani}, U. and {Bellazzini}, M. and {Berihuete}, A. and {Bertone}, S. and {Bianchi}, L. and {Bienaym{\'e}}, O. and {Blanco-Cuaresma}, S. and {Boch}, T. and {Boeche}, C. and {Bombrun}, A. and {Borrachero}, R. and {Bossini}, D. and {Bouquillon}, S. and {Bourda}, G. and {Bragaglia}, A. and {Bramante}, L. and {Breddels}, M.~A. and {Bressan}, A. and {Brouillet}, N. and {Br{\"u}semeister}, T. and {Brugaletta}, E. and {Bucciarelli}, B. and {Burlacu}, A. and {Busonero}, D. and {Butkevich}, A.~G. and {Buzzi}, R. and {Caffau}, E. and {Cancelliere}, R. and {Cannizzaro}, G. and {Cantat-Gaudin}, T. and {Carballo}, R. and {Carlucci}, T. and {Carrasco}, J.~M. and {Casamiquela}, L. and {Castellani}, M. and {Castro-Ginard}, A. and {Charlot}, P. and {Chemin}, L. and {Chiavassa}, A. and {Cocozza}, G. and {Costigan}, G. and {Cowell}, S. and {Crifo}, F. and {Crosta}, M. and {Crowley}, C. and {Cuypers}, J. and {Dafonte}, C. and {Damerdji}, Y. and {Dapergolas}, A. and {David}, P. and {David}, M. and {de Laverny}, P. and {De Luise}, F. and {De March}, R. and {de Martino}, D. and {de Souza}, R. and {de Torres}, A. and {Debosscher}, J. and {del Pozo}, E. and {Delbo}, M. and {Delgado}, A. and {Delgado}, H.~E. and {Di Matteo}, P. and {Diakite}, S. and {Diener}, C. and {Distefano}, E. and {Dolding}, C. and {Drazinos}, P. and {Dur{\'a}n}, J. and {Edvardsson}, B. and {Enke}, H. and {Eriksson}, K. and {Esquej}, P. and {Eynard Bontemps}, G. and {Fabre}, C. and {Fabrizio}, M. and {Faigler}, S. and {Falc{\~a}o}, A.~J. and {Farr{\`a}s Casas}, M. and {Federici}, L. and {Fedorets}, G. and {Fernique}, P. and {Figueras}, F. and {Filippi}, F. and {Findeisen}, K. and {Fonti}, A. and {Fraile}, E. and {Fraser}, M. and {Fr{\'e}zouls}, B. and {Gai}, M. and {Galleti}, S. and {Garabato}, D. and {Garc{\'\i}a-Sedano}, F. and {Garofalo}, A. and {Garralda}, N. and {Gavel}, A. and {Gavras}, P. and {Gerssen}, J. and {Geyer}, R. and {Giacobbe}, P. and {Gilmore}, G. and {Girona}, S. and {Giuffrida}, G. and {Glass}, F. and {Gomes}, M. and {Granvik}, M. and {Gueguen}, A. and {Guerrier}, A. and {Guiraud}, J. and {Guti{\'e}rrez-S{\'a}nchez}, R. and {Haigron}, R. and {Hatzidimitriou}, D. and {Hauser}, M. and {Haywood}, M. and {Heiter}, U. and {Helmi}, A. and {Heu}, J. and {Hilger}, T. and {Hobbs}, D. and {Hofmann}, W. and {Holland}, G. and {Huckle}, H.~E. and {Hypki}, A. and {Icardi}, V. and {Jan{\ss}en}, K. and {Jevardat de Fombelle}, G. and {Jonker}, P.~G. and {Juh{\'a}sz}, {\'A}. L. and {Julbe}, F. and {Karampelas}, A. and {Kewley}, A. and {Klar}, J. and {Kochoska}, A. and {Kohley}, R. and {Kolenberg}, K. and {Kontizas}, M. and {Kontizas}, E. and {Koposov}, S.~E. and {Kordopatis}, G. and {Kostrzewa-Rutkowska}, Z. and {Koubsky}, P. and {Lambert}, S. and {Lanza}, A.~F. and {Lasne}, Y. and {Lavigne}, J. -B. and {Le Fustec}, Y. and {Le Poncin-Lafitte}, C. and {Lebreton}, Y. and {Leccia}, S. and {Leclerc}, N. and {Lecoeur-Taibi}, I. and {Lenhardt}, H. and {Leroux}, F. and {Liao}, S. and {Licata}, E. and {Lindstr{\o}m}, H.~E.~P. and {Lister}, T.~A. and {Livanou}, E. and {Lobel}, A. and {L{\'o}pez}, M. and {Managau}, S. and {Mann}, R.~G. and {Mantelet}, G. and {Marchal}, O. and {Marchant}, J.~M. and {Marconi}, M. and {Marinoni}, S. and {Marschalk{\'o}}, G. and {Marshall}, D.~J. and {Martino}, M. and {Marton}, G. and {Mary}, N. and {Massari}, D. and {Matijevi{\v{c}}}, G. and {Mazeh}, T. and {McMillan}, P.~J. and {Messina}, S. and {Michalik}, D. and {Millar}, N.~R. and {Molina}, D. and {Molinaro}, R. and {Moln{\'a}r}, L. and {Montegriffo}, P. and {Mor}, R. and {Morbidelli}, R. and {Morel}, T. and {Morris}, D. and {Mulone}, A.~F. and {Muraveva}, T. and {Musella}, I. and {Nelemans}, G. and {Nicastro}, L. and {Noval}, L. and {O'Mullane}, W. and {Ord{\'e}novic}, C. and {Ord{\'o}{\~n}ez-Blanco}, D. and {Osborne}, P. and {Pagani}, C. and {Pagano}, I. and {Pailler}, F. and {Palacin}, H. and {Palaversa}, L. and {Panahi}, A. and {Pawlak}, M. and {Piersimoni}, A.~M. and {Pineau}, F. -X. and {Plachy}, E. and {Plum}, G. and {Poggio}, E. and {Poujoulet}, E. and {Pr{\v{s}}a}, A. and {Pulone}, L. and {Racero}, E. and {Ragaini}, S. and {Rambaux}, N. and {Ramos-Lerate}, M. and {Regibo}, S. and {Reyl{\'e}}, C. and {Riclet}, F. and {Ripepi}, V. and {Riva}, A. and {Rivard}, A. and {Rixon}, G. and {Roegiers}, T. and {Roelens}, M. and {Romero-G{\'o}mez}, M. and {Rowell}, N. and {Royer}, F. and {Ruiz-Dern}, L. and {Sadowski}, G. and {Sagrist{\`a} Sell{\'e}s}, T. and {Sahlmann}, J. and {Salgado}, J. and {Salguero}, E. and {Sanna}, N. and {Santana-Ros}, T. and {Sarasso}, M. and {Savietto}, H. and {Schultheis}, M. and {Sciacca}, E. and {Segol}, M. and {Segovia}, J.~C. and {S{\'e}gransan}, D. and {Shih}, I. -C. and {Siltala}, L. and {Silva}, A.~F. and {Smart}, R.~L. and {Smith}, K.~W. and {Solano}, E. and {Solitro}, F. and {Sordo}, R. and {Soria Nieto}, S. and {Souchay}, J. and {Spagna}, A. and {Spoto}, F. and {Stampa}, U. and {Steele}, I.~A. and {Steidelm{\"u}ller}, H. and {Stephenson}, C.~A. and {Stoev}, H. and {Suess}, F.~F. and {Surdej}, J. and {Szabados}, L. and {Szegedi-Elek}, E. and {Tapiador}, D. and {Taris}, F. and {Tauran}, G. and {Taylor}, M.~B. and {Teixeira}, R. and {Terrett}, D. and {Teyssandier}, P. and {Thuillot}, W. and {Titarenko}, A. and {Torra Clotet}, F. and {Turon}, C. and {Ulla}, A. and {Utrilla}, E. and {Uzzi}, S. and {Vaillant}, M. and {Valentini}, G. and {Valette}, V. and {van Elteren}, A. and {Van Hemelryck}, E. and {van Leeuwen}, M. and {Vaschetto}, M. and {Vecchiato}, A. and {Veljanoski}, J. and {Viala}, Y. and {Vicente}, D. and {Vogt}, S. and {von Essen}, C. and {Voss}, H. and {Votruba}, V. and {Voutsinas}, S. and {Walmsley}, G. and {Weiler}, M. and {Wertz}, O. and {Wevers}, T. and {Wyrzykowski}, {\L}. and {Yoldas}, A. and {{\v{Z}}erjal}, M. and {Ziaeepour}, H. and {Zorec}, J. and {Zschocke}, S. and {Zucker}, S. and {Zurbach}, C. and {Zwitter}, T.},
        title = "{Gaia Data Release 2. Summary of the contents and survey properties}",
      journal = {A\&A},
     keywords = {catalogs, astrometry, techniques: radial velocities, stars: fundamental parameters, stars: variables: general, minor planets, asteroids: general, Astrophysics - Astrophysics of Galaxies, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2018,
        month = aug,
       volume = {616},
          eid = {A1},
        pages = {A1},
          doi = {10.1051/0004-6361/201833051},
archivePrefix = {arXiv},
       eprint = {1804.09365},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018A&A...616A...1G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gillessen2017,
       author = {{Gillessen}, S. and {Plewa}, P.~M. and {Eisenhauer}, F. and {Sari}, R. and {Waisberg}, I. and {Habibi}, M. and {Pfuhl}, O. and {George}, E. and {Dexter}, J. and {von Fellenberg}, S. and {Ott}, T. and {Genzel}, R.},
        title = "{An Update on Monitoring Stellar Orbits in the Galactic Center}",
      journal = {ApJ},
     keywords = {astrometry, black hole physics, Galaxy: center, Galaxy: fundamental parameters, techniques: high angular resolution, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = mar,
       volume = {837},
       number = {1},
          eid = {30},
        pages = {30},
          doi = {10.3847/1538-4357/aa5c41},
archivePrefix = {arXiv},
       eprint = {1611.09144},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...837...30G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{LinShu1964,
       author = {{Lin}, C.~C. and {Shu}, Frank H.},
        title = "{On the Spiral Structure of Disk Galaxies.}",
      journal = {ApJ},
         year = 1964,
        month = aug,
       volume = {140},
        pages = {646},
          doi = {10.1086/147955},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1964ApJ...140..646L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Krone-Martins2014A&A...561A..57K,
       author = {{Krone-Martins}, A. and {Moitinho}, A.},
        title = "{UPMASK: unsupervised photometric membership assignment in stellar clusters}",
      journal = {A\&A},
     keywords = {open clusters and associations: general, open clusters and associations: individual: Haner 10, methods: data analysis, methods: statistical, open clusters and associations: individual: Haner 16, open clusters and associations: individual: Czernik 29, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = "2014",
        month = "Jan",
       volume = {561},
          eid = {A57},
        pages = {A57},
          doi = {10.1051/0004-6361/201321143},
archivePrefix = {arXiv},
       eprint = {1309.4471},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014A&A...561A..57K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Lindblad1938,
       author = {{Lindblad}, Bertil},
        title = "{On the theory of spiral structure in the nebulae.}",
      journal = {ZAP},
         year = 1938,
        month = jan,
       volume = {15},
        pages = {124},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1938ZA.....15..124L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{LiuPang2019,
       author = {{Liu}, Lei and {Pang}, Xiaoying},
        title = "{A Catalog of Newly Identified Star Clusters in Gaia DR2}",
      journal = {ApJS},
     keywords = {catalogs, galaxies: star clusters: general, methods: data analysis, open clusters and associations: general, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = dec,
       volume = {245},
       number = {2},
          eid = {32},
        pages = {32},
          doi = {10.3847/1538-4365/ab530a},
archivePrefix = {arXiv},
       eprint = {1910.12600},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJS..245...32L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Monteiro2020,
       author = {{Monteiro}, H. and {Dias}, W.~S. and {Moitinho}, A. and {Cantat-Gaudin}, T. and {L{\'e}pine}, J.~R.~D. and {Carraro}, G. and {Paunzen}, E.},
        title = "{Fundamental parameters for 45 open clusters with Gaia DR2, an improved extinction correction and a metallicity gradient prior}",
      journal = {MNRAS},
     keywords = {open clusters and associations: general, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2020,
        month = sep,
       volume = {499},
       number = {2},
        pages = {1874-1889},
          doi = {10.1093/mnras/staa2983},
archivePrefix = {arXiv},
       eprint = {2009.11834},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.499.1874M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Roberts1969,
       author = {{Roberts}, W.~W.},
        title = "{Large-Scale Shock Formation in Spiral Galaxies and its Implications on Star Formation}",
      journal = {ApJ},
         year = 1969,
        month = oct,
       volume = {158},
        pages = {123},
          doi = {10.1086/150177},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1969ApJ...158..123R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Reid2019,
       author = {{Reid}, M.~J. and {Menten}, K.~M. and {Brunthaler}, A. and {Zheng}, X.~W. and {Dame}, T.~M. and {Xu}, Y. and {Li}, J. and {Sakai}, N. and {Wu}, Y. and {Immer}, K. and {Zhang}, B. and {Sanna}, A. and {Moscadelli}, L. and {Rygl}, K.~L.~J. and {Bartkiewicz}, A. and {Hu}, B. and {Quiroga-Nu{\~n}ez}, L.~H. and {van Langevelde}, H.~J.},
        title = "{Trigonometric Parallaxes of High-mass Star-forming Regions: Our View of the Milky Way}",
      journal = {ApJ},
     keywords = {Milky Way, Milky Way dynamics, Milky Way rotation, Trigonometric parallax, Star formation, Gravitational wave sources, 1054, 1051, 1059, 1713, 1569, 677, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = nov,
       volume = {885},
       number = {2},
          eid = {131},
        pages = {131},
          doi = {10.3847/1538-4357/ab4a11},
archivePrefix = {arXiv},
       eprint = {1910.03357},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...885..131R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Reid2016,
       author = {{Reid}, M.~J. and {Dame}, T.~M.},
        title = "{On the Rotation Speed of the Milky Way Determined from H I Emission}",
      journal = {ApJ},
     keywords = {Galaxy: kinematics and dynamics, Galaxy: fundamental parameters, Galaxy: structure, ISM: atoms, Astrophysics - Astrophysics of Galaxies},
         year = 2016,
        month = dec,
       volume = {832},
       number = {2},
          eid = {159},
        pages = {159},
          doi = {10.3847/0004-637X/832/2/159},
archivePrefix = {arXiv},
       eprint = {1608.03886},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...832..159R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Reid2014,
       author = {{Reid}, M.~J. and {Menten}, K.~M. and {Brunthaler}, A. and {Zheng}, X.~W. and {Dame}, T.~M. and {Xu}, Y. and {Wu}, Y. and {Zhang}, B. and {Sanna}, A. and {Sato}, M. and {Hachisuka}, K. and {Choi}, Y.~K. and {Immer}, K. and {Moscadelli}, L. and {Rygl}, K.~L.~J. and {Bartkiewicz}, A.},
        title = "{Trigonometric Parallaxes of High Mass Star Forming Regions: The Structure and Kinematics of the Milky Way}",
      journal = {ApJ},
     keywords = {Galaxy: fundamental parameters, Galaxy: kinematics and dynamics, Galaxy: structure, gravitational waves, parallaxes, stars: formation, Astrophysics - Galaxy Astrophysics},
         year = 2014,
        month = mar,
       volume = {783},
       number = {2},
          eid = {130},
        pages = {130},
          doi = {10.1088/0004-637X/783/2/130},
archivePrefix = {arXiv},
       eprint = {1401.5377},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...783..130R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Soubiran2018,
       author = {{Soubiran}, C. and {Cantat-Gaudin}, T. and {Romero-G{\'o}mez}, M. and {Casamiquela}, L. and {Jordi}, C. and {Vallenari}, A. and {Antoja}, T. and {Balaguer-N{\'u}{\~n}ez}, L. and {Bossini}, D. and {Bragaglia}, A. and {Carrera}, R. and {Castro-Ginard}, A. and {Figueras}, F. and {Heiter}, U. and {Katz}, D. and {Krone-Martins}, A. and {Le Campion}, J. -F. and {Moitinho}, A. and {Sordo}, R.},
        title = "{Open cluster kinematics with Gaia DR2}",
      journal = {A\&A},
     keywords = {stars: kinematics and dynamics, Galaxy: kinematics and dynamics, open clusters and associations: general, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = nov,
       volume = {619},
          eid = {A155},
        pages = {A155},
          doi = {10.1051/0004-6361/201834020},
archivePrefix = {arXiv},
       eprint = {1808.01613},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018A&A...619A.155S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Shu2016,
       author = {{Shu}, Frank H.},
        title = "{Six Decades of Spiral Density Wave Theory}",
      journal = {ARA\&A},
         year = 2016,
        month = sep,
       volume = {54},
        pages = {667-724},
          doi = {10.1146/annurev-astro-081915-023426},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ARA&A..54..667S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Shu1972,
       author = {{Shu}, Frank H. and {Milione}, Vincenzo and {Gebel}, William and {Yuan}, C. and {Goldsmith}, D.~W. and {Roberts}, W.~W.},
        title = "{Galactic Shocks in an Interstellar Medium with Two Stable Phases}",
      journal = {ApJ},
         year = 1972,
        month = may,
       volume = {173},
        pages = {557},
          doi = {10.1086/151444},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1972ApJ...173..557S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sim2019,
       author = {{Sim}, Gyuheon and {Lee}, Sang Hyun and {Ann}, Hong Bae and {Kim}, Seunghyeon},
        title = "{207 New Open Star Clusters within 1 kpc from Gaia Data Release 2}",
      journal = {Journal of Korean Astronomical Society},
     keywords = {open cluster and associations: general, catalogs, methods: data analysis, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = oct,
       volume = {52},
        pages = {145-158},
          doi = {10.5303/JKAS.2019.52.5.145},
archivePrefix = {arXiv},
       eprint = {1907.06872},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019JKAS...52..145S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Xu2006,
       author = {{Xu}, Y. and {Reid}, M.~J. and {Zheng}, X.~W. and {Menten}, K.~M.},
        title = "{The Distance to the Perseus Spiral Arm in the Milky Way}",
      journal = {Science},
     keywords = {ASTRONOMY, Astrophysics},
         year = 2006,
        month = jan,
       volume = {311},
       number = {5757},
        pages = {54-57},
          doi = {10.1126/science.1120914},
archivePrefix = {arXiv},
       eprint = {astro-ph/0512223},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006Sci...311...54X},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lepine2017,
       author = {{L{\'e}pine}, Jacques R.~D. and {Michtchenko}, Tatiana A. and {Barros}, Douglas A. and {Vieira}, Ronaldo S.~S.},
        title = "{The Dynamical Origin of the Local Arm and the Sun's Trapped Orbit}",
      journal = {ApJ},
     keywords = {Galaxy: disk, kinematics and dynamics, solar neighborhood, structure, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = jul,
       volume = {843},
       number = {1},
          eid = {48},
        pages = {48},
          doi = {10.3847/1538-4357/aa72e5},
archivePrefix = {arXiv},
       eprint = {1705.04381},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...843...48L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Junqueira2013,
       author = {{Junqueira}, T.~C. and {L{\'e}pine}, J.~R.~D. and {Braga}, C.~A.~S. and {Barros}, D.~A.},
        title = "{A new model for gravitational potential perturbations in disks of spiral galaxies. An application to our Galaxy}",
      journal = {A\&A},
     keywords = {Galaxy: kinematics and dynamics, Galaxy: structure, galaxies: spiral, galaxies: bulges, Astrophysics - Astrophysics of Galaxies},
         year = 2013,
        month = feb,
       volume = {550},
          eid = {A91},
        pages = {A91},
          doi = {10.1051/0004-6361/201219769},
archivePrefix = {arXiv},
       eprint = {1212.3312},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013A&A...550A..91J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{JohnsonSoderblom1987,
       author = {{Johnson}, Dean R.~H. and {Soderblom}, David R.},
        title = "{Calculating Galactic Space Velocities and Their Uncertainties, with an Application to the Ursa Major Group}",
      journal = {AJ},
     keywords = {A Stars, Computational Astrophysics, Eclipsing Binary Stars, Spatial Distribution, Stellar Motions, Velocity Distribution, Radial Velocity, Star Clusters, Stellar Parallax, Astronomy, STARS: PROPER-MOTION, CLUSTERS: OPEN},
         year = 1987,
        month = apr,
       volume = {93},
        pages = {864},
          doi = {10.1086/114370},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1987AJ.....93..864J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Schonrich2010,
       author = {{Sch{\"o}nrich}, Ralph and {Binney}, James and {Dehnen}, Walter},
        title = "{Local kinematics and the local standard of rest}",
      journal = {MNRAS},
     keywords = {stars: kinematics, Galaxy: disc, Galaxy: fundamental parameters, Galaxy: kinematics and dynamics, solar neighbourhood, Astrophysics - Astrophysics of Galaxies},
         year = 2010,
        month = apr,
       volume = {403},
       number = {4},
        pages = {1829-1833},
          doi = {10.1111/j.1365-2966.2010.16253.x},
archivePrefix = {arXiv},
       eprint = {0912.3693},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010MNRAS.403.1829S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Villegas2015,
       author = {{P{\'e}rez-Villegas}, Angeles and {G{\'o}mez}, Gilberto C. and {Pichardo}, B{\'a}rbara},
        title = "{The galactic branches as a possible evidence for transient spiral arms}",
      journal = {MNRAS},
     keywords = {MHD, Galaxy: disc, Galaxy: kinematics and dynamics, Galaxy: structure, galaxies: spiral, galaxies: structure, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2015,
        month = aug,
       volume = {451},
       number = {3},
        pages = {2922-2932},
          doi = {10.1093/mnras/stv1157},
archivePrefix = {arXiv},
       eprint = {1505.04327},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.451.2922P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lepine2011,
       author = {{L{\'e}pine}, J.~R.~D. and {Cruz}, P. and {Scarano}, S., Jr. and
         {Barros}, D.~A. and {Dias}, W.~S. and {Pomp{\'e}ia}, L. and
         {Andrievsky}, S.~M. and {Carraro}, G. and {Famaey}, B.},
        title = "{Overlapping abundance gradients and azimuthal gradients related to the spiral structure of the Galaxy}",
      journal = {MNRAS},
     keywords = {stars: kinematics and dynamics, Galaxy: abundances, Galaxy: evolution, Galaxy: structure, Astrophysics - Astrophysics of Galaxies},
         year = 2011,
        month = oct,
       volume = {417},
       number = {1},
        pages = {698-708},
          doi = {10.1111/j.1365-2966.2011.19314.x},
archivePrefix = {arXiv},
       eprint = {1106.3137},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011MNRAS.417..698L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Monteiro2017,
       author = {{Monteiro}, H. and {Dias}, W.~S. and {Hickel}, G.~R. and {Caetano}, T.~C.},
        title = "{The OPD photometric survey of open clusters II. robust determination of the fundamental parameters of 24 open clusters}",
      journal = {NA},
     keywords = {(Galaxy:) Open clusters, Associations:general, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = feb,
       volume = {51},
        pages = {15-27},
          doi = {10.1016/j.newast.2016.08.001},
archivePrefix = {arXiv},
       eprint = {1608.03010},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017NewA...51...15M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Burton_Gordon1978,
   author = {{Burton}, W.~B. and {Gordon}, M.~A.},
    title = "{Carbon monoxide in the Galaxy. III - The overall nature of its distribution in the equatorial plane}",
  journal = {A\&A},
 keywords = {CARBON MONOXIDE, GALACTIC NUCLEI, GALACTIC RADIATION, HYDROGEN CLOUDS, INTERSTELLAR GAS, MOLECULAR ROTATION, ABUNDANCE, ASTRONOMICAL MODELS, EMISSION SPECTRA, HYDROGEN ATOMS, MOLECULAR SPECTRA, STOCHASTIC PROCESSES},
     year = 1978,
    month = feb,
   volume = 63,
    pages = {7-27},
   adsurl = {http://adsabs.harvard.edu/abs/1978A%26A....63....7B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Clemens1985,
   author = {{Clemens}, D.~P.},
    title = "{Massachusetts-Stony Brook Galactic plane CO survey - The Galactic disk rotation curve}",
  journal = {ApJ},
 keywords = {CARBON MONOXIDE, GALACTIC ROTATION, INTERSTELLAR GAS, MILKY WAY GALAXY, ANGULAR VELOCITY, GALACTIC NUCLEI, H II REGIONS, RADIAL VELOCITY},
     year = 1985,
    month = aug,
   volume = 295,
    pages = {422-428},
      doi = {10.1086/163386},
   adsurl = {http://adsabs.harvard.edu/abs/1985ApJ...295..422C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fich_Blitz_Stark1989,
   author = {{Fich}, M. and {Blitz}, L. and {Stark}, A.~A.},
    title = "{The rotation curve of the Milky Way to 2 R(0)}",
  journal = {ApJ},
 keywords = {GALACTIC ROTATION, MILKY WAY GALAXY, SPECTROPHOTOMETRY, CARBON MONOXIDE, ERROR ANALYSIS, H II REGIONS, NORTHERN SKY, PLANETARY NEBULAE},
     year = 1989,
    month = jul,
   volume = 342,
    pages = {272-284},
      doi = {10.1086/167591},
   adsurl = {http://adsabs.harvard.edu/abs/1989ApJ...342..272F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Reid_etal2019,
       author = {{Reid}, M.~J. and {Menten}, K.~M. and {Brunthaler}, A. and
         {Zheng}, X.~W. and {Dame}, T.~M. and {Xu}, Y. and {Li}, J. and
         {Sakai}, N. and {Wu}, Y. and {Immer}, K. and {Zhang}, B. and
         {Sanna}, A. and {Moscadelli}, L. and {Rygl}, K.~L.~J. and
         {Bartkiewicz}, A. and {Hu}, B. and {Quiroga-Nu{\~n}ez}, L.~H. and
         {van Langevelde}, H.~J.},
        title = "{Trigonometric Parallaxes of High-mass Star-forming Regions: Our View of the Milky Way}",
      journal = {ApJ},
     keywords = {Milky Way, Milky Way dynamics, Milky Way rotation, Trigonometric parallax, Star formation, Gravitational wave sources, 1054, 1051, 1059, 1713, 1569, 677, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = nov,
       volume = {885},
       number = {2},
          eid = {131},
        pages = {131},
          doi = {10.3847/1538-4357/ab4a11},
archivePrefix = {arXiv},
       eprint = {1910.03357},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...885..131R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rastorguev_etal2017,
       author = {{Rastorguev}, A.~S. and {Utkin}, N.~D. and {Zabolotskikh}, M.~V. and
         {Dambis}, A.~K. and {Bajkova}, A.~T. and {Bobylev}, V.~V.},
        title = "{Galactic masers: Kinematics, spiral structure and the disk dynamic state}",
      journal = {Astrophysical Bulletin},
     keywords = {Astrophysics - Astrophysics of Galaxies, 85A05, J.2},
         year = 2017,
        month = apr,
       volume = {72},
       number = {2},
        pages = {122-140},
          doi = {10.1134/S1990341317020043},
archivePrefix = {arXiv},
       eprint = {1603.09124},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017AstBu..72..122R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{Binney,
       author = {{Binney}, James and {Tremaine}, Scott},
        title = "{Galactic dynamics}",
         year = 1987,
         publisher = {Princeton, N.J. : Princeton University Press, c1987},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1987gady.book.....B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gustafsson,
       author = {{Gustafsson}, Bengt and {Church}, Ross P. and {Davies}, Melvyn B. and {Rickman}, Hans},
        title = "{Gravitational scattering of stars and clusters and the heating of the Galactic disk}",
      journal = {A\&A},
     keywords = {Galaxy: kinematics and dynamics, open clusters and associations: individual: M 67, Sun: evolution, stars: formation, Astrophysics - Astrophysics of Galaxies},
         year = 2016,
        month = sep,
       volume = {593},
          eid = {A85},
        pages = {A85},
          doi = {10.1051/0004-6361/201423916},
archivePrefix = {arXiv},
       eprint = {1605.02965},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016A&A...593A..85G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

